On the Fine-Grained Complexity of the Unbounded SubsetSum and the Frobenius Problem

Consider positive integral solutions $x \in \mathbb{Z}^{n+1}$ to the equation $a_0 x_0 + \ldots + a_n x_n = t$. In the so called unbounded subset sum problem, the objective is to decide whether such a solution exists, whereas in the Frobenius problem, the objective is to compute the largest $t$ such that there is no such solution. In this paper we study the algorithmic complexity of the unbounded subset sum, the Frobenius problem and a generalization of the problems. More precisely, we study pseudo-polynomial time algorithms with a running time that depends on the smallest number $a_0$ or respectively the largest number $a_n$. For the parameter $a_0$, we show that all considered problems are subquadratically equivalent to $(min,+)$-convolution, a fundamental algorithmic problem from the area of fine-grained complexity. By this equivalence, we obtain hardness results for the considered problems (based on the assumption that an algorithm with a subquadratic running time for $(min,+)$-convolution does not exist) as well as algorithms with improved running time. The proof for the equivalence makes use of structural properties of solutions, a technique that was developed in the area of integer programming. In case of the complexity of the problems parameterized by $a_n$, we present improved algorithms. For example we give a quasi linear time algorithm for the Frobenius problem as well as a hardness result based on the strong exponential time hypothesis.

==> outtakes.tex <==

\begin{algorithm} \label{alg:subsetsum}
\caption{Solving \subsetsum}
\begin{enumerate}
    \item Compute for $i \leq a_n/a_0$ the sets
    \begin{align*}
        S^{(i)} = S^{(i-1)} + S^{(i-1)} \cap I^{(1)}
    \end{align*}
    \item Set 
    \begin{align*}
        A^{(1)} = S^{(a_n/a_0)}.
    \end{align*}
    \item Compute sets $A^{(2^i)}$ iteratively while $|A^{(2^i)}| < a_{n}$ by
    \begin{align*}
        A^{(2^i)} = (A^{(2^{i-1})} + A^{(2^{i-1})} + S) \cap I^{(2^i)}.
    \end{align*}
    Let $L$ be the index with $|A^{(2^i)}| = a_{n}$
    \item
        \begin{align*}
            A^{(k+2^i)} = (A^{(2^i)} + A + S) \cap I^{(k+2^i)}
        \end{align*}
    \item Let $I^{(j)}$ be the interval with $t \in I^{(j)}$. Compute $A^{(j)}$ by
    \begin{align*}
        A^{(j)} = \sum_{i \in Bin(i)} A^{(2^i)} \cap I^{(j)},
    \end{align*}
    where $Bin(j)$ is the set of indices with a $1$ in the binary encoding of $j$, i.e. $\sum_{i \in Bin(i)} 2^i = j$.
    \item If $j> 2^L$ or $t \in A^{(j)}$ return $t$ is feasible otherwise return that (\ref{IP1}) is infeasible.
\end{enumerate}
\end{algorithm}


\begin{algorithm} 
\caption{Solving \frobenius}
\begin{enumerate}
    \item Compute the sets $A^{(2^0)}, A^{(2^1)}, \ldots , A^{(2^R)}$ as in steps (1)--(3) of Algorithm~\ref{alg:subsetsum}, where $R$ is the smallest number with $|A^{2^R}| = n$.
    \item Use a binary search in the interval $[2^{R-1},2^R)$ to determine the largest index $f \in [2^{R-1},2^R)$ with $|A^{(f)}| < n$ by using Algorithm~\ref{alg:subsetsum} repeatedly to determine the sets $A^{(i)}$.
    \item Return the Frobenius number $F = f \cdot a_n + r$, where $r = \max A^{f}$.
\end{enumerate}
\end{algorithm}


\begin{algorithm}
    \State{index := $2^{R-1}$}
    \For{$i=1$ to $R-1$}
    {
        \State{$A := A + A^{(2^{R-1-i})} + S \cap I$}
        \If{$|A|<n$}{
            \State{index = index + $2^{R-1-i}$}     
            }
    }
\end{algorithm}

\begin{algorithm}\caption{Efficient Binary Search}
\begin{algorithmic}
    \STATE{$M := 2^{R-1}$}
    \FOR{$i=R-2$ \textbf{downto} $0$}{
        \STATE{$A^{(M+2^{i})} = (A^{(M)} + A^{(2^i)} + S) \cap I^{(M+2^{i})}$}
        \COMMENT{blabla}
        \IF {$|A^{(M+2^{i})}| < a_n$} 
            \STATE $M := M + 2^i$
        \ENDIF
    }
    \ENDFOR
    \RETURN $M$
\end{algorithmic}
\end{algorithm}


\begin{tcolorbox}
    \textsc{Boolean Convolution}
    
    \textbf{Input:} Sequences $(a[i])_{i=0}^{n-1}$ and $(b[i])_{i=1}^n$ with $a[i],b[i] \in \{0,1 \}$ for all $1 \leq i \leq n$.\\
    \textbf{Objective:} Compute a sequence $(c[i])_{i=0}^{n-1}$, such that \begin{align*}
        c[k] = \bigvee_{i+j=k} (a[i] \land b[j]) .
    \end{align*}
\end{tcolorbox}


\item Compute iteratively for $i \leq \lceil \log a_n/a_0 \rceil$ the sets $S^{(i)}$ starting with $S^{(1)} := S$
    \begin{align*}
        S^{(2^i)} = (S^{(2^{i-1})} + S^{(2^{i-1})}) \cap I^{(1)}
    \end{align*}
    \item Set $A^{(1)} := S^{(2^{\lceil \log a_n/a_0 \rceil})}$.
    
    
Therefore $A^{(1)}$ is computed correctly in step (1) and (2) of the algorithm as each feasible target value consists of a sum of at most $\lfloor a_n/a_0 \rfloor$ elements of $S$ as otherwise a sum of more than $\frac{a_n}{a_0}$ items would exceed $a_n$. Therefore, 
\begin{align*}
    A^{(1)} = \big( \underbrace{S + \ldots + S}_{\lfloor a_n/a_0 \rfloor} \big) \cap I^{(1)} = S^{(2^{\lceil \log a_n/a_0 \rceil})} \cap I^{(1)}.
\end{align*}

Let $\Tilde{n}$ be the number of items after removing items $a_i$ with $a_i \equiv a_j \bmod a_0$ and $a_i > a_j$. Note that those items are redundant as $a_j$ can be represented by $a_i$ and multiples of item $a_0$.


\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
        Problem & Running Time - $a_0$ & Running Time - $a_n$\\
        \hline 
        \subsetsum & $O(\log \log (a_0) \cdot MinConv(a_0))$ & $O(a_n \log a_n \cdot \log (\frac{a_n}{a_0}+\frac{F}{a_n}))$\\
         \frobenius& $O(\log \log (a_0) \cdot MinConv(a_0))$ & $O(a_n \log a_n \cdot \log (\frac{a_n}{a_0}+\frac{F}{a_n}))$\\
         \allvalues & $O(\log \log (a_0) \cdot MinConv(a_0))$ & $O(a_{n}^{3/2} \log^{1/2} a_n)$
    \end{tabular}
    \caption{Algorithmic Results}
    \label{tab:my_label}
\end{table}
